QPack: Quantum Approximate Optimization Algorithms as universal benchmark for quantum computers

In this paper, we present QPack, a universal benchmark for Noisy Intermediate-Scale Quantum (NISQ) computers based on Quantum Approximate Optimization Algorithms (QAOA). Unlike other evaluation metrics in the field, this benchmark evaluates not only one, but multiple important aspects of quantum computing hardware: the maximum problem size a quantum computer can solve, the required runtime, as well as the achieved accuracy. The applications MaxCut, dominating set and traveling salesman are included to provide variation in resource requirements. This will allow for a diverse benchmark that promotes optimal design considerations, avoiding hardware implementations for specific applications. We also discuss the design aspects that are taken in consideration for the QPack benchmark, with critical quantum benchmark requirements in mind. An implementation is presented, providing practical metrics. QPack is presented as a hardware agnostic benchmark by making use of the XACC library. We demonstrate the application of the benchmark on various IBM machines, as well as a range of simulators.

==> bench_config_old.tex <==
\section{Benchmark configuration}
\label{sec:config}
In this chapter the details on the benchmark configuration are discussed. This includes a discussion on selecting a classical optimizer for finding the optimal $\bm{\beta}$ and $\bm{\gamma}$ parameter, as well as details on the quantum implementation of the QAOA algorithms.

\subsection{Parameter optimization}
\label{sec:param_opt}

This section explores the strategies to optimally determine the $\bm{\beta}$ and $\bm{\gamma}$ parameters. The optimization of these parameters is considered to be the main bottleneck of QAOA \cite{sarkar2020quaser}, and the selection of the optimizer could make or break the application. The optimization is a single objective real-parameter optimization and is done classically. Many algorithms have been developed for this problem. Critical parameters for choosing a classical optimizer are as follows:

\begin{itemize}
    \item number of parameters to optimize
    \item size of the problem instance
    \item smoothness of the objective function
    \item number of local optima
\end{itemize}

\textbf{Gradient-based optimization algorithms}\\
Gradient-based optimization uses the gradient of the problem function to find a (local) optimum. Gradient-based optimizers converge generally faster than gradient-free ones and would therefore be favorable \cite{opt_ch3}. However, gradient-based optimization only works well on smooth functions and is prone to getting stuck in local optima. Due to the dependency on smooth functions, any function that is either discontinuous or noisy will cause problems for the optimization. In the case that a smooth function is available, the problem of local minima could be averted by choosing multiple starting points and running the optimization multiple times or in parallel if possible. This, however, increases the computational complexity and choosing an efficient algorithm for the starting value is not trivial. Often random points are chosen, but a more efficient algorithm based on the Discrete Fourier Transform (DFT) is presented by \cite{Zhou_2020} but is not open-source.

%The explored Gradient-Based algorithms are:
%\begin{enumerate}[label*=\arabic*.]
%    \item Newton method
%    \item Quasi-Newton method
%    \begin{enumerate}[label*=\arabic*.]
%        \item BFGS
%        \item square root BFGS
%        \item DFP update
%        \item limited memory BFGS
%        \item non-linear Conjugate Gradient
%    \end{enumerate}
%    \item Gradient Descent
%    \begin{enumerate}[label*=\arabic*.]
%        \item Batch
%        \item Stochastic
%        \item Mini-batch
%    \end{enumerate}
%    \item Steepest Descent
%    \item Trust region
%\end{enumerate}

\textbf{Gradient-free optimization algorithms}\\
Gradient-free algorithms do not depend on the gradient of the function, as the name suggests. This means that these algorithms can be applied to objective functions that are noisy, discrete or discontinuous \cite{opt_ch6}. Gradient-free methods can be more resilient with respect to local minima, depending on the algorithm. The downside of these algorithms is that these generally take more computation time or more iterations.

\subsubsection{Problem instances}
The objective function is evaluated with the above mentioned critical aspects, in order to find the optimization algorithm that fits best. The objective functions are considered in general and not per individual problem. The reason for this will become apparent in the evaluation.

\textbf{Number of parameters}: For all problems, the number of parameters are $2 p$: $\beta_p$ and $\gamma_p$ for each QAOA iteration $p$. Optionally, $p$ can be taken as a parameter as well, but since publications show that QAOA is most effective in low depth, i.e. low $p$, this parameter is expected not to contribute significantly. Generally a value for $p$ is chosen beforehand (e.g. Crooks \cite{crooks2018performance} shows that $p \geq 8$ is required to outperform the Goemans-Williamson algorithm) after which $\beta$ and $\gamma$ are optimized. Theoretically, an optimizer would increase $p$ to infinite as this would give the best results. In practice, $p$ can optionally be included as well, as performance is likely to decrease with higher circuit dept on quantum hardware.

\textbf{Problem size}: The problem size is expected to grow larger with the development of larger quantum devices in terms of qubits. Especially for qubit inefficient implementations such as TSP, problem size is a significant factor.

\textbf{Smoothness of objective function}: The smoothness of the objective function is expected to differ per problem type. However, due to the probabilistic nature of the results, as well as noise in quantum hardware, the objective function is never smooth in practice.

\textbf{Local optima}: The presence of local optima is dependent on each individual problem, but due to noise in quantum hardware, local optima might still occur. Local optima might not be as strong as local minima inherent to the objective function. This could give room to optimizers that have some trouble escaping from strong local optima.


\subsection{Selection of optimizer} \label{sec:c_opt}
\noindent Considering how all QAOA problem instances will suffer from noise, discontinuities and local optima, no gradient-based optimizer can be applied. From the gradient-free algorithms the following are considered:
\\

\textbf{Nelder-Mead Simplex}: Nelder-Mead is efficient for non-smooth objective functions. It is, however, not very efficient for 10 or more design variables \cite{lec_notes_opt}. Considering that only $2\times p$ variables are optimized, the Nelder-Mead optimizer fits well for low-depth QAOA. Nelder-Mead is also more resilient with regard to local optima compared to other local optimizers.\\

\textbf{Genetic Algorithms}: Genetic algorithms generally require many function evaluations, but are applicable to multi-objective optimizations \cite{lec_notes_opt}. Genetic algorithms are not well-suited, since QAOA problems only have one objective function. The large number of iterations are therefore inefficient.\\

\textbf{Simulated Annealing (SA)}: Simulated annealing has more freedom than other gradient-free optimization algorithms, but comparison to other algorithms shows that the computation per iteration of SA is less efficient. Alternatively, SA could be accelerated with VQE, but the performance is not yet adequately explored and will be more demanding for the quantum hardware. Potentially, this could be used in the future when quantum hardware is more mature and scalable.\\

\textbf{Particle swarm optimization (PSO)}: Particle swarm optimization can converge fast, has a short computational time and has very few parameters to adjust \cite{lec_notes_opt}. The downsize is that it is prone to get trapped in local optima, especially with complex problems \cite{optmization_PSO}. Since large problem instances need to be considered with regards to scalability, PSO might not be suited for QAOA. PSO could be considered for problem instances with no inherent local optima (i.e. local optima due to noise). Unfortunately, it could be difficult to tune initial parameters for PSO. Considering that QAOA should be applied to multiple different problems, tuning the parameters could create a bottleneck. PSO could be considered an option for similar problems and a custom PSO parameterization. A custom PSO could be considered for the Ising model, with seemingly no inherent local optima \cite{pagano2020quantum}, but not for the more popular and more developed MaxCut  \cite{Khairy2019ReinforcementLF}.\\

\textbf{Symmetric Rank-1 Update Method (SR1)}: The SR1 method is not a gradient-free algorithm, but is included for special cases. SR1 uses a first-order derivative, as opposed to a second-order derivative like the Newton method. This means that the smoothness requirement on the objective function is less strict. In the case that the hardware has sufficiently low noise and multiple measurements per iteration are performed, the SP1 method might be applicable. The main difficulty, is that it is subjective to how smooth an objective function needs to be for SP1 to perform well, as no clear comparison is done between noise levels in objective functions and performance of the algorithm. It would also require the objective function to be evaluated, meaning it would be unclear per implementation if the algorithm works well. Quasi-Newton methods such as SP1 and the Broyden–Fletcher–Goldfarb–Shanno algorithm (BFGS) only work for finding local minima. This means that if multiple local minima exist in the solution landscape, the global minima might not be found. With this observation in mind, SR1 can only be applied to objective functions with only one minimum and would require extensive evaluation of the objective function. Another Quasi-Newton method that is commonly used is the BFGS algorithm, but as long as the problem field has a limit constraint (in this case $\gamma, \beta \in [0, 2\pi]$), SR1 converges faster. \\

More state-of-the-art algorithms exist, as competitions in the field of single objective real-parameters optimization are organized by IEEE yearly (CEC Real-Parameter Optimization Competitions) but since the winning algorithms have not been found as either open-source or a library, the winning algorithms are not considered for application. Regardless, the best algorithm for low dimensions was found to be UMOEA \cite{CEC}.\\

From the evaluated optimizers, Nelder-Mead is considered the best fit for QAOA. Numerical comparison of classical optimizers \cite{num_eval} show that in terms of performance, BFGS and Nelder-Mead differ very little in run-time and find identical results in sufficiently smooth functions. This raises the argument that if the objective function is sufficiently smooth, Nelder-Mead could be used as well and no custom optimizer needs to be applied. This saves development time for the application. PSO or SR1 could be considered only for very special cases. For the general case, UMOEA could be implemented to possibly further improve performance.

==> benchmark_outline.tex <==
\section{Benchmark outline}\label{sec:outline}
\noindent Having determined the algorithm to base the benchmark on, the outline of QPack is presented for implementation. In order to properly evaluate the performance of a quantum hardware implementation in practice, the following aspects need to be considered:

\begin{enumerate}%[label*=\arabic*.]
    \item runtime
    \begin{enumerate}%[label*=\arabic*.]
        \item Classic computation
        \item Classic to quantum connection
        \item Quantum computation
    \end{enumerate}
    \item Outcome accuracy / best approximation error
    %\begin{enumerate}[label*=\arabic*.]
        %\item 

    \item Performance scaling\\
\end{enumerate}

\textbf{runtime}: The runtime of an application is an obvious parameter to measure. Classically, apart from the functionality, this is the main parameter measured as it separates implementations on their practical performance. Since the quantum hardware is only practical in hybrid configuration, both the classical and quantum hardware need to be evaluated. While the quantum speedup should be most significant to the performance, for QAOA optimization it was found that the classical optimizer is crucial to the performance of the QAOA optimization \cite{sarkar2020quaser}. Determining the performance of the classical hardware is therefore essential.  For this reason the following runtimes need to be observed:
\begin{itemize}
    \item Overall runtime   
    \item runtime classical hardware    
    \item Connection between classical and quantum hardware    
    \item Preprocessing/placing and routing
    \item runtime quantum hardware   \\ 
\end{itemize}

The connection between quantum and classical hardware might very well be significant to the overall performance. Multiple calls need to be made to the quantum hardware in QAOA. Since quantum computing is a Compute as a Service (CaaS) in current implementations, the way the connection is organized as well as the relative slow internet connection can be crucial. In cases that the implementation is organized with a local classical computer sending instructions to the remote quantum computer, most time will be lost by this connection. A more mature implementation would be both a remote classical computer and a remote quantum computer, which share a faster local connection. By explicitly measuring these parameters, much more crucial information is learned about the bottleneck of an implementation. As the benchmark does not optimize quantum instructions to suit specific hardware, the performance of the compiler will be reflected as well and will translate to the number of instructions generated and how the quantum circuit is scheduled. Other bottlenecks on the implementation could include: number of calls to quantum hardware from classical hardware and time required per quantum instruction.\\

\textbf{Best approximation error}: QAOA can only approximate an optimal solution. While this is dependent on parameter $p$ and the classical optimization strategy, it will also be dependent on the hardware. The qubit quality will determine the noise in a system and will determine $p$ \cite{alam2019analysis} and can significantly decrease performance. Furthermore, gate error and finite coherence time can introduce significant bounds on $p$, limiting not only compensation for noise, but also place significant bounds on scaling. Another effect on the accuracy could be $\ket{0}$ bias \cite{guerrero2020solving}. This means that the states are more likely to be measured as a logical $0$ rather than a logical $1$, skewing the outcome and effecting the accuracy. The approximation can be evaluated in multiple ways.\\

1. The benchmark will be run on the hardware with optimal parameter $p$, determined iteratively. This way the maximum achievable accuracy can be found by comparing it to the solution of an exact algorithm. This has as downside that multiple runs will be required to find the correct parameter, and increasing $p$ will increase the runtime, which might not be properly reflected this way. If the runtime of the implementation is however presented for only the optimal parameter, it will likely better reflect how the optimization would be implemented in practice. This way a decision will be made for the trade-off between speed and accuracy, favoring accuracy. The difficult part is that, in the case that there are no bounds on $p$, $p$ might grow to infinity, approaching exact calculation. Recent research show that increasing $p$ will not always improve accuracy \cite{niu2019optimizing} and will have a practical limit.\\

2. The other method is to test for, e.g., $p \in \{1,2,3,4\}$ and compare these results. This way the runtime will not be determined by the choice of $p$, but the accuracy will reflect the quality of the quantum hardware. This will require more interpretation, as the accuracy shown will not be the optimal accuracy, but shows how the accuracy will be for low iterations of $p$. The difficulty in this approach lies in determining how $p$ scales for larger problem sizes. The size of $p$ is expected to grow with the problem size, but at which rate is not yet determined. Some research suggest that QAOA will only be practical for low depth (e.g. $p$=2) and therefore eliminated this issue.\\ %!!! cite
From both approaches, the latter appears to be the most fair and with fewer issues, but demands an explanation on how to interpret the results.\\

Alternatively, an approach can be taken where the accuracy is evaluated for a predetermined runtime. This however requires that the runtime will not be constant for each problem size as the runtime is expected to grow. Determining a starting point for the run time as well as how this will progress for the problem size is nontrivial. For this reason, method 1 is preferred.\\

\textbf{Success probability}: The probability of success is another measure of the quality of the quantum hardware. Preferably, the best approximation error of the QAOA implementation reaches $0$ for some amount of runs. The probability of success can be determined by the percentage of runs that achieve the optimal solution and will, much like the best approximation error, reflect the quality of the quantum hardware. This method however requires that the implementation can in fact find the optimal solution, rendering the previous method obsolete.

\textbf{Performance scaling}: With concerns as bounds on $p$ and scaling issues, it is important to give insight on how the benchmark performance scales for larger problem sizes. By determining the runtime for increasing problem size, the scaling performance can be reviewed. Similarly, it can be evaluated on how the accuracy or success probability decreases for larger problem sizes.

While this benchmark is focused on quantum hardware, it could be extended to quantum simulators, evaluating runtime and memory consumption. This could give valuable insight to developers to find the optimal simulator to work with.

\subsection{Implementation}
%figure: https://arxiv.org/pdf/1812.01041.pdf
\noindent The implementation of the benchmark will require universality, in the sense that it should run on every quantum computer. The XACC library \cite{XACC} is suited for this task and will be used to implement the benchmark. The benchmark will require multiple steps. Multiple problems need to be tested in order to show that the hardware is not optimized for a single problem. The problems that will be tested are:
\begin{itemize}
    \item MaxCut problem (MCP)
    \item Traveling salesman problem (TSP)
    \item Dominating set problem (DSP) \\
    \end{itemize}
These problems have been chosen due to the effectiveness of QAOA on them, and their technological readiness level as explored in Section \ref{sec:QTRL}. These problems will then need to be tested for increasing problem size, until the quantum hardware is unable to find a solution. This could be either due to not having enough qubits, or having a too low chance of finding the optima ($< 50\%$). The QAOA runs themselves will need multiple runs to determine the success rate and average runtime and accuracy. The solutions found by the QAOA optimization, need to be compared to a pre-computed answer using a classical exact algorithm. If the hardware supports larger circuit depth, the QAOA algorithm can be adjusted to a maximum $p$. As theoretically the best found solution is always larger or equal to solutions found for smaller QAOA depth $p$, a maximum value can be found when the found solution does not improve or diminishes. Diminishing of the solution indicates that no larger circuit depth is possible. This search to a maximum $p$ can be included as an additional step for the benchmark to find the best accuracy of the QAOA implementation. The maximum circuit depth and width of quantum hardware will translate to maximum resources per available memory for a quantum simulator. \\

To give insight on $\ket{0}$ bias, a trivial circuit can be run beforehand. The measurements will indicate if there is a bias. The implementation of QAOA will be done using a classical optimizer which is further explored in Section \ref{sec:c_opt_meas}.

\begin{figure}[ht]
    \centering
    \includegraphics[width = 0.3\textwidth]{figures/flowchart_benchmark.pdf}
    \caption{Flowchart for proposed benchmark}
    \label{fig:flowchart}
\end{figure}

As the benchmark needs to be reproducible, the configuration of the problems must be predetermined. Akshay et al. \cite{Akshay_2020} show that the performance of QAOA in terms of configurations is mainly due to the density (e.g. in a graph: the number of edges with respect to the number of vertices). As the benchmark needs to scale to an undefined problem size, the problems configurations cannot be hard-coded. In the proposed benchmark, the density will remain the same, to make the performance predetermined. This can for example be achieved by a bounded connectivity. Alternatively, a set of connections can be predetermined and a regular structure will be applied and scaled. This however is not necessarily representative of practical applications. The number of "shots" for a single QAOA iteration will range between 10 and 100, as these give the best results \cite{Zhou_2020}. The number of iterations to achieve an estimation of the accuracy must be further analyzed. Expected is that the estimation will saturate towards a maximum reliability. A lower bound must be determined for this reliability. Determining the parameter $p$ is also not trivial. There are arguments that the accuracy of QAOA will not grow for $p>2$ \cite{Marshall_2020}, but others argue that e.g. a minimum of $p \geq 8$ is required for the MaxCut application to compete with classical approaches \cite{crooks2018performance}. Determining $p$, possibly dependent on the application will require further numerical analysis.

The outline for QPack is given schematically in Figure \ref{fig:flowchart}. Here an initial $\ket{0}$ bias test is done, and the QAOA applications are run for increasing problem sizes. The benchmark will stop if for all applications the maximum problem size has been reached. The maximum is determined if \textbf{a)} not enough qubits are available, or \textbf{b)}, the probability of finding the correct result falls below 50\%. The cut-off limit of 50\% has been chosen as below this threshold, re-iterating the algorithm will not produce better results. Some design choices can be made to make sure the benchmark is as complete as possible. First of all, the generation of problems can be done every iteration of the QAOA optimization. It would be fairest to create a new configuration of the problem, as certain configurations might be easier to optimize and might give an unfair advantage. This however will require longer computation times for the benchmark itself. The number of QAOA runs is also debatable. More runs will give a better average, but a limit must be set to limit the runtime. Another interesting addition would be adding both weighted and unweighted problems for the problems. This can show if the hardware is optimized with e.g. using parameter "sensitive" edges \cite{entropica}. This solution would preferably be implemented by the benchmark, but requires too much information about the hardware, which should be abstracted. A quantum instruction compiler would be tasked to implement the qubit SWAPs required for this method. A further concern is that the benchmark should allow for parallelism. With the current size of quantum hardware, it is unlikely that this will be fully exploited in practice. However, as quantum hardware will scale up, there should be support to apply the parallelism. For the suggested Nelder-Mead classical optimization algorithm, a parallel variant has been developed \cite{ozaki2019accelerating, dennis1988parallel, lee2007parallel}. This will allow the use of more quantum resources to compute smaller problems.


% section results for different p

% section results for different problem complexities

% section comparison different hamiltonians

%Zaid: we need to add some initial measurements !!! ??? !!!

%Zaid: add a time planning per week till end of January to finish a first version! !!! ??? !!!

%week 51: edit details current benchmark plan % ✔
%         explore and measure classical optimizer for numerical results 
%week 52: classical optimizer results and figures
        %finding optimal p for problems
%week 53: explore effect of problem density on performance, determine configuration for benchmark

%week 1 : classical optimizers, results and comparison % ✔
%week 2 : optimal p for selected optimizer, effect of problem density
%week 3 : implement different problem hamiltonians
%week 4 : process results to report
   %      finishing report
  %       review


%notes
%interesting to compare to approximation ratios of heuristic solvers?
%\cite{Shaydulin_2019} finds p>4 to do worse
%\cite{Zhou_2020} p=5 > p=1
%\cite{Zhou_2020}: NM slightly outperforms BFGS, even with initial point generation
%multiple runs for average runtime
%optional: find for each problem size optimal p

%scoring:   inpractical:    (accuracy) * 1/runtime
%           practical:      (success probability) * 1/runtime || scaling coeff * max problemsize

%Quantum Computing Hardware Implementation Points (Q-CHIP)
%Quantum Performance Optimization Index in Normalised Terms (Q-POINT)
%quantum hardware index
%Quantum Hardware implementation 

%number of shots is not optimal, trade-off runs and smoothness/accuracy (will smoothness reduce classical optimizer?)
%Settings on NM/BFGS were tailored to assure proper execution and assure convergence
%Randomized implementation of BFGS/NM is not implemented due to the already high run time cost. If even higher cost is needed, the algorithms cannot compete against other algorithms.
%Accuracy only considers how close the found expectation value is to the expectation value of a fine grid search (brute force). This does not evaluate beta and gamma values, meaning that while the result is close, it might be stuck in a local optimum. This method was chosen, as even in local optima a value very close or even equal to the best value can be found, but if a local optima far from the brute force solution is found in terms of beta and gamma, the accuracy will be unjustly represented.


==> measurements.tex <==
\section{Configuration measurements}
\label{sec:measurements}
In this section, measurements of the different classical optimizer options and the different QAOA implementations are presented. These measurements were done using Qiskit qasm simulator, to show relative performances of classical parameter optimizers and QAOA applications.

\subsection{Measurements of classical optimizers}\label{sec:c_opt_meas}

\noindent In Appendix \ref{sec:param_opt}, a preliminary study of various classical optimizers was done. In this section, various promising classical optimization algorithms will be applied for increasing problem size to compare the runtime performance and accuracy. Apart from Nelder-Mead and BFGS, which are both discussed in Appendix \ref{sec:param_opt}, other optimization algorithms available in open-source libraries are presented as well. The list of tested optimizers is:

\begin{enumerate}%[label*=\arabic*.]
    \item Local optimizers
    \begin{enumerate}%[label*=\arabic*.]
        \item Nelder-Mead
        \item BFGS
        \item NEWUOA
        \item BOBYQA
        \item COBYLA
    \end{enumerate}
    \item Global optimizers
    \begin{enumerate}%[label*=\arabic*.]
        \item Dual annealing
        \item SHGO (simplicial homology global optimization)
        \item ISRES
        \item MLSL / MLSL\_LDS (Multi-Level Single-Linkage, low-discrepancy sequence)
        \item DIRECT (DIviding RECTangles)
        \item StoGO
    \end{enumerate}
\end{enumerate}

These algorithms were implemented in Python using either SciPy or the NL-Opt library \cite{NLOpt}. Some of these algorithms are not included in the following results, as either no convergence was found (due to various reasons) or if the optimization had such a long runtime that it cannot be considered a contender in comparison to other algorithms. The algorithms included in this list are: \\

\begin{itemize}
    \item Dual annealing
    \item NEWUOA
    \item BOBYQA
    \item ISRES
    \item MLSL / MLSL\_LDS
    \item DIRECT
    \item StoGO
\end{itemize}

Perhaps with different implementations, these algorithms could be used for QAOA optimization. In the case of dual annealing, it was clear that convergence could be found, but takes significantly longer than other tested optimization algorithms. The MLSL implementation suffers from searching for every local optima (which can be very significant with noisy QAOA results). A variant of MLSL might work for QAOA, but with the current implementation no convergence could be found in reasonable time. \\

\begin{figure}[h]
    \centering
    \includegraphics[width=0.55\linewidth]{figures/timing_data.pdf}
    \caption{Data of runtime measurements fitted to exponential functions. Any number in the legend indicates the convergence tolerance, which is default if not indicated.}
    \label{fig:timing_opt}
\end{figure}


The runtime measurements were done on MaxCut problems with 3 to 23 nodes, as above 20 nodes run times become very large and simulating many data points becomes too time-consuming. The QAOA algorithm is implemented using Qiskit for the Qasm simulator \cite{quasm} The MaxCut problems are randomly configured, but have the same number of edges as nodes to maintain the problem complexity. The results are shown in Figure \ref{fig:timing_opt}. The data is fitted to an exponential function, as the obtained data shows a clear exponential growth. In this figure, it can be seen that the Nelder-Mead algorithms which was expected to perform best, is in fact the slowest from the selected algorithms in practice. SHGO, COBYLA and BOBYQA perform much better in terms of runtime, with SHGO being the fastest. \\

\begin{figure}
    \centering
    \includegraphics[width=0.55\linewidth]{figures/relative_acc.pdf}
    \caption{Optimizer Accuracy compared to Dual-Annealing for the same problem graph. Here a lower relative accuracy shows a more accurate algorithm. A negative value shows that the tested algorithm outperforms the Dual-Annealing algorithm. R COBYLA here indicated the COBYLA algorithm using multiple randomized starting points.}
    \label{fig:acc_opt}
\end{figure}

For the accuracy measurements, the different algorithms solve the same MaxCut problem for different sizes and the best expectation values are compared. Preferably, a fine grid search (brute force) is implemented to compare the results to, but this proved to be too time consuming to collect data, even for small problems. In Figure \ref{fig:acc_opt}, the found expected values are compared to the value found by the Dual-Annealing algorithm. Dual-Annealing was chosen, since it was a slower global optimizer, but allowed for reasonable computing times and expecting that this would outperform the faster algorithms. The difference in accuracy is calculated as $\textit{relative accuracy} = \frac{\textit{DA expectation value} - \textit{tested algorithm expectation value} }{\textit{DA expectation value}}$. The results however show that Dual-Annealing does always find better solutions and is often outperformed. The \textit{beta} and \textit{gamma} parameters are not compared, as different local minima might find values very close to the optimal value. The results show clearly that COBYLA using randomized starting points outperforms other algorithms, indicating that a hybrid approach finds the best solutions. This, however, significantly increases the search time. For the single algorithm approaches, Nelder-Mead finds the best expectation values, presenting a trade-off between accuracy and time. It should be noted that for larger problem sizes, the expectation values are much closer and it is expected that for scaling purposes it is better to choose a faster algorithm such as COBYLA, BOBYQA of SHGO. Some parameters such as the number of the QAOA iterations or the convergence tolerance are not optimized as this is expected to give minimal change to the results with respect to the comparison.\\

Considering the found results in terms of accuracy and runtime, a hybrid approach could be applied. Heuristics such as random starting points combined with a local optimizer are often applied, to counter the local optimizer of getting trapped in local optima. Another implementation is the use of a (fast) global optimizer with a more accurate local optimizer. In the case of optimizer QAOA parameters, using a fast algorithm such as SHGO combined with e.g. Nelder-Mead of BFGS would be a good approach. This approach needs to be be investigated with respect to which global optimizer accuracy specification (which translates to runtime), will outperform random starting points for a similar runtime. Furthermore, many combinations are possible of both local and global optimizers. These combinations are worth examining to find better runtimes for a set accuracy and vice versa.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Measurements of applications} \label{sec:app_measurements}
\noindent A common downside of computer benchmarks is that hardware vendors are tempted to tailor their systems to excel in the particular benchmarks. We have therefore included multiple applications to the QPack benchmark. Next to the MaxCut problem (MCP), the dominating set problem (DSP) and the traveling salesman problem (TSP) have been included. In this section, the details on the QAOA implementation will be discussed, as well as the effect on the measured performance.

The MaxCut application has been examined in detail in Appendix \ref{sec:MaxCut}. The QAOA implementation requires the following gates for $n$ vertices and $m$ edges(or clauses) and $p$ QAOA iterations: \\

\begin{tabular}{|c|c|}
\hline
    Gate type  & \# gates\\
    \hline
    Hadamard & $n$ \\
    CNOT & $2m \cdot p$ \\
    RZ & $m \cdot p$ \\
    RX & $n \cdot p$ \\
    \hline
\end{tabular}\\

From the applications explored, MaxCut QAOA requires the least gates and is therefore expected to run best on NISQ era devices. MaxCut will result in the smallest circuit depth and does not require additional ancilla qubits. \\

The QAOA for DSP is implemented according to the algorithm provided by Nicholas Guerrero \cite{guerrero2020solving}. This implementation uses logical OR gates, which can be implemented using CNOT gates and ancilla qubits. The number of required ancillas and CNOT per logical OR depends on the number of input qubits k. The number of required ancillas is k-1. The implementation by Guerrero uses the logical OR to control a RY gate. This OR-controlled RY gate requires one additional ancilla as target qubit. As the ancillas can be re-used, the ancillas per circuit add up to k ancillas, with $2 \leq k \leq n$. The logical 2-OR uses 3 CNOT gates, as depicted in Figure \ref{fig:2OR}. These 2-OR gates can be combined to a n-input logical OR. For n inputs, this n-OR is implemented as: \\
\begin{lstlisting}
qc = QuantumCircuit(2*n)
qc.append(ORGate, [0, 1, n])
for i in range(2, n):
    qc.append(ORGate, [i, n+i-2, n+i-1])
qc.crz(gamma, 2*n-2, 2*n-1)
for i in range(n, 2, -1):
    qc.append(ORGate, [n-i-1, 2*n-2-i, 2*n-1-i])
qc.append(ORGate, [0, 1, n])

\end{lstlisting}
\begin{figure}[h]
    \centering
    \includegraphics[clip, trim=5cm 8.5cm 5cm 3cm, width=0.3\linewidth]{figures/2-OR.pdf}
    \caption{Implementation of a 2-input logical OR using CNOT gates.}
    \label{fig:2OR}
\end{figure}

The circuit can be implemented using the following resources (at most): \\


\begin{tabular}{|c|c|}
    \hline
    Gate type &  \# gates\\
    \hline
    Hadamard & $n$ \\
    X & $2m \cdot p$ \\
    CNOT & $((6n-5) \cdot m) \cdot p$ \\
    RZ & $m \cdot p$ \\
    RX & $n \cdot p$ \\
    \hline
\end{tabular}\\
$n$ qubits are inititialised in superposition, using $n$ Hadamard gates. Inverted controlled RZ-gates and OR-controlled RZ-gates are used to implement the $m$ clauses \cite{guerrero2020solving}. The $n$ RX gates are then applied to the $n$ qubits. Excluding the initialization, this is repeated for $p$ iterations.


The DSP QAOA implementation uses similar, but significantly more resources than the MCP implementation. The DSP implementation uses $(6n-7)\cdot m \cdot p$ more CNOT gates and $2n \cdot p$ additional Pauli-X gates. This requires quantum computers to support larger circuit depth, but also more ancilla qubits and better CNOT mapping. The additional CNOT requirement will reflect the qubit connectivity of the quantum hardware implementation, as well as the handling of qubit SWAPS (if required) by the hardware scheduler. \\

The TSP QAOA implementation is a much more demanding quantum algorithm and with the current implementation also uses different resources. The implementation is done according to this github blog: \textbf{\texttt{\url{https://lucaman99.github.io/new_blog/2020/mar16.html}}} \cite{tsp_git} which is one of the few examples of a clear implementation. The author however indicates that the state preparation is sub optimal and is therefore altered to suit the algorithm better. The TSP algorithm, as other QAOA algorithm, consists of a state preparation, a mixer Hamiltonian and a cost Hamiltonian. Whereas the MCP and DSP QAOA need $n$ to $2n$ qubits for n vertices, this implementation uses $n^2$ qubits. Other variations exist, such as presented by Ruan et al. \cite{ruan_tsp}, using $m$ qubits, which is at most $n(n-1)/2$ qubits for a fully connected graph. This implementation will be considered a future improvement. This however means that the 
current implementation requires significantly more qubits compared to MCP and DSP. \\

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/singleplot_app.pdf}
    \caption{Runtime comparison for MCP, DSP and TSP QAOA applications, implemented in Qiskit, plotted in a single figure (only 100 QAOA runs were done for comparison)}
    \label{fig:app_runtime}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/multiplot_app.pdf}
    \caption{Runtime comparison for MCP, DSP and TSP QAOA applications, implemented in Qiskit plotted in separate figures for detail}
    \label{fig:app_runtime_2}
\end{figure}

For the state preparation $n$ binary strings of length $n$ are required with a Hamming weight of 2. The superposition of all possible strings with a set Hamming weight is called a Dicke state \cite{Dicke}. In the TSP implementation a Dicke state preparation is applied on each row of $n$ qubits for Hamming weight 2, using the implementation by Bärtschi and Eidenbenz \cite{Dicke_state_prep}. The cost and mixer Hamiltonian are left unchanged. Considering the significant cost of both the Dicke state preparation and the QAOA cycles, it worth mentioning the costs separately. The gate counts are provided in the following tables: \\

\begin{multicols}{2}
\begin{tabular}{|c|c|}
\hline
 \multicolumn{2}{|c|}{Dicke State Preparation Cost} \\
    \hline
    Gate type &  \# gates\\
    \hline
    Hadamard & $8n(n-2)$ \\
    $T/T^\dagger$ & $49n(n-2)$ \\
    CNOT & $(31n-28)n$ \\
    RY & $(6n - 10)n $ \\
    X & $2n$ \\
    \hline
\end{tabular}

\begin{tabular}{|c|c|}
\hline
 \multicolumn{2}{|c|}{TSP QAOA cycles Cost} \\
    \hline
    Gate type &  \# gates\\
    \hline
    RZ & $n^2 \cdot p$ \\
    RZZ & $\frac{n^2-n}{2} \cdot p$ \\
    RXX & $2n \cdot p$ \\
    RYY & $2n \cdot p$ \\
    \hline
\end{tabular}
\end{multicols}

This shows that while not only the circuit cost is significantly higher, many different gates are used. This will avoid fine tuning of quantum computers on solely Hademard, CNOT, RX and RZ Gates. To compare the impact of the different applications, a runtime comparison was done. The applications are implemented using the SHGO classical optimizer. The results in Figures \ref{fig:app_runtime} and \ref{fig:app_runtime_2} show that the runtime corresponds to the increase of circuit depth and required qubits as expected. Note that Figures \ref{fig:app_runtime} and \ref{fig:app_runtime_2} do not show large problem sizes for DSP and TSP as the larger problem sizes result in simulator memory issues. Despite the smaller data range, the difference in runtimes can be clearly distinguished.


==> theory_complexity.tex <==
\section{Practical application of problems}
\label{sec:prac_app}
This section will explore potential fields, where QAOA could be implemented to achieve significant speedup over classical algorithms. A brief introduction to the theoretical problems will be given, with their practical applications. For each problem, the current QAOA implementations will be reviewed in terms of complexity and approximation accuracy.

\subsection{A brief recap of complexity theory}
Computational problems can be sorted by their time complexity. This refers to the computational resources required to solve the problem for $n$ inputs. Often, big-$O$ notation is used to describe the resources required for the worst-case scenario, while big-$\Omega$ notation is used for best-case scenarios. If both the worst-case and best-case scenarios match, big-$\Theta$ notation can be used. A graph of common time complexities is given in Figure \ref{fig:complex}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/complexities.png}
    \caption{A graph of common time complexities \cite{hidary}}
    \label{fig:complex}
\end{figure}

Problems can be subdivided in classes, depending on their complexity. These classes consist of:\\
\textbf{P}: \quad Problems of polynomial time complexity range from $O(1)$ to $O(n^p)$, with $p \in \mathbbm{N}$ fixed \cite{hidary}, and can be solved efficiently with classical computers.\\
\textbf{NP}: \quad NP stands for Non-deterministic polynomial time and is used to classify decision problems. These problems initially determine a solution in a Non-deterministic way (a guess), and is then verified in polynomial time \cite{algorithms}. \\
\textbf{NP-complete}: \quad Problem 'A' is considered \textbf{NP-complete} if 'A' is in \textbf{NP} and if all \textbf{NP} problems can be reduced to 'A' in polynomial time. If the problem is only known to be in \textbf{NP}, it is considered \textbf{NP-hard} \cite{hidary}.  \\

\textbf{BPP}: \quad Bounded-error probabilistic polynomial time are a class of decision problems, to which a randomized algorithm can find the solution in polynomial time with probability $p \geq \frac{1}{2}$ \cite{hidary}. The problem set includes \textbf{P} and parts of \textbf{NP}, but not all. A visualization of the complexity classes is given in figure \ref{fig:complexity_diagram}.

\textbf{BQP}: \quad Bounded-error quantum polynomial time is the quantum analogue tot the BPP complexity class \cite{hidary, BQP}. Again, the quantum algorithm has a probability of 
$p \geq \frac{1}{2}$ to find the correct answer in polynomial time.

\textbf{EQP}: Exact quantum polynomial time is the set of problems that can be found in polynomial time by a quantum algorithm with probability $p = 1$ \cite{hidary}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.50\linewidth]{figures/complexity_space.png}
    \caption{A Venn-diagram of the complexity classes \cite{BQP}}
    \label{fig:complexity_diagram}
\end{figure}

In 1971, Stephen Cook proved that the satisfiability problem is \textbf{NP-complete} \cite{Cook}. The year after that, Richard Karp expanded the list of \textbf{NP-complete} problems to the well known list of Karp's 21 \textbf{NP-complete} problems \cite{conf/coco/Karp72}.  An overview of the problems is given in Figure \ref{fig:karp}. This list was established by showing that these 20 additional problems can be reduced to the satisfiability problem in polynomial time. Any problem can only be \textbf{NP-complete} if it is a decision problem. Finding the optimization for such a problem is \textbf{NP-hard}. The solutions to these problems have been approximated by classical algorithms to a limited accuracy (in polynomial time). QAOA improves on these algorithms by making the guess more accurate while remaining within polynomial time complexity. From here on, some of the optimizations to Karp's 21 problems will be discussed, including practical applications. Not all 21 problems will be discussed, as only the problems will be considered where a QAOA implementation has been designed to improve on the classical counterpart. Other \textbf{NP-hard} problems, not directly related to Karp's 21 problems, will be included as well.
The satisfiability problem, as described in section is a problem where is Boolean clause needs to be satisfied. All of Karp's problems can be reduced to a satisfiability problem in polynomial time. The satisfiability problem is commonly denoted as Max-Sat. A $k$-Max-Sat is a satisfiability problem where each clause is limited to $k$ variables. The QAOA algorithm is applied to the \textit{approximation} of NP-hard problems, as optimization of \textbf{NP} problems are \textbf{NP-hard}. This means that, while a solution might be found with QAOA, this only has a probability of finding the solution and is therefore contained in \textbf{BQP} complexity. Note that QAOA can not approximate a solution for all \textbf{NP-hard} problems, but a subset of similar structured problems. As discussed above, theoretically QAOA could find a solution with probability $p=1$. But since this is not demonstrated to be achievable in polynomial time, it cannot be considered as \textbf{EQP} complexity. 

\begin{figure}[h]
    \centering
    %\includegraphics[clip, trim=3cm 20cm 10cm 3cm, width=0.8\linewidth]{figures/karp21.pdf}
    \includegraphics[width=0.8\linewidth]{figures/Karps_21_problems.pdf}
    \caption{Karp's 21 problems, with the reduction relations given as a tree diagram \cite{conf/coco/Karp72}}
    \label{fig:karp}
\end{figure}

\subsection{The QAOA implementations to the problems} \label{sec:problems}
This section explores QAOA algorithms applied to various NP-hard problems.
\subsubsection{Graph partition}
In the graph partition problem,  a graph ($V,E$) is divided into partitions with the objective to minimize edges in order to simplify graph analysis. This problem can be applied to VLSI circuit design as the first step of the physical design \cite{kahng2011vlsi}. A QAOA implementation has been presented by Ruan et al. \cite{ruan2020quantum}, with a general QAOA scheme for linear inequality constraints.

Problems with a linear equality constraint have the characteristic that their constraints are represented as:
\begin{equation}
    \mathbf{A} \cdot \mathbf{x} = \mathbf{b}
\end{equation}

With $\mathbf{A}$ being a $m \times n$ matrix for $m$ constraints and $n$ components, $\mathbf{x}$ the solution vector of length $n$ and $\mathbf{b}$ a vector of length $m$. Such a problem translates to a constraint function of \cite{ruan2020quantum} :
\begin{equation}
    f(\mathbf{x}) = \sum_k \mathbf{c}_k \cdot \mathbf{x}_k 
\end{equation}

In this scheme, the $B$ operator is defined as follows:
\begin{equation} \label{eq:qwalk}
    B = \sum_{\mathbf{x,x'}\in \Omega, \mathbf{d(x,x')=2}} \ket{x}\bra{x'}+\ket{x'}\bra{x}
\end{equation}
Here $\mathbf{d(x,x')}$ is the Hamming distance between solution $\mathbf{x}$ and $\mathbf{x'}$. This way of encoding the $B$ operator is derived from a random quantum walk, where positions and orders of "1's" are swapped.  In the case of the graph partition problem, the $B$ operator is rewritten by Hadfield and Hen \cite{Hadfield_2019, Hen_2016} to encode the constraints as:
\begin{equation} \label{eq:b_alt}
    B = - \sum_i^n (\sigma_i^x \sigma_{i+1}^x + \sigma_i^y \sigma_{i+1}^y)
\end{equation}

Both solutions differ in outcome. The probability distribution from equation \eqref{eq:qwalk} is more accurate than the implementation from \eqref{eq:b_alt}, and does not generate redundant subgraphs \cite{ruan2020quantum}.

\subsubsection{Packing (knapsack)}
The packing problem, or knapsack problem, aims to fill a resource as full as possible. As example, given a knapsack with a limited capacity, fill it with as much elements as the capacity allows. Ruan et al. implement QAOA on this problem for multiprocessors with a similar solution as mentioned in the previous section. The Hamiltonian for this implementation is given by:
\begin{equation}
    C = - \sum_{x=0}^{2^{mn}-1} \max \{ \sum_{k=in}^{(i+1)n-1} t_{k \mod n}x_k \} \ket{x}\bra{x} \text{ for }i = 0, ... , (m-1) \textbf{,}
\end{equation}
where $t$ is the execution time for a task. De la Grand'rive and Hullo also published a paper on this particular problem, with a different approach aimed at an implementation for battery revenue optimization for micro-grids \cite{delagrandrive2019knapsack}. In their paper, a 'relaxed' approach is presented, using a linear penalty as opposed to a quadratic penalty to improve upon the adiabatic approach \cite{coffey2017adiabatic}. The algorithm proposed, consists of four subroutines: Cost calculation, Constraint testing, Penalty dephasing and Reinitialisation. In terms of time complexity, the classical algorithm for the knapsack problem runs in $O(\frac{n^3}{\epsilon})$ for $\epsilon$-estimation \cite{delagrandrive2019knapsack}.  The implementation presented can run with a qubit depth of $O(p(\log_2(n))^3)$, meaning that it achieves a $p$-polylogarithmic complexity in $n$. The number of ancillary qubits required for this algorithm is $O(n \log_2(n)$.
Another paper published on this problem is by Roch et al. \cite{roch2020cross} and uses a cross entropy hyper parameter optimization. With this method, the penalty values are optimized. An enhancement for $p = 1$ and $p=2$ of more than 100\% is claimed compared to the method of Hadfield et al. \cite{Hadfield_2019}.
Ruan et al. expanded on the packing problem by adding arbitrary constraints. Since the previous method of changing the Hamming distance does not apply, they present a \textit{star graph} method. Their results are claimed to be similar to classical optimization algorithms in terms of accuracy, but not much about complexity or performance is presented.

